Will it Unblend?

Natural language processing systems often struggle with out-of-vocabulary (OOV) terms, which do not appear in training data. Blends, such as "innoventor", are one particularly challenging class of OOV, as they are formed by fusing together two or more bases that relate to the intended meaning in unpredictable manners and degrees. In this work, we run experiments on a novel dataset of English OOV blends to quantify the difficulty of interpreting the meanings of blends by large-scale contextual language models such as BERT. We first show that BERT's processing of these blends does not fully access the component meanings, leaving their contextual representations semantically impoverished. We find this is mostly due to the loss of characters resulting from blend formation. Then, we assess how easily different models can recognize the structure and recover the origin of blends, and find that context-aware embedding systems outperform character-level and context-free embeddings, although their results are still far from satisfactory.

==> tab_surface_tags.tex <==
\begin{table}
    \small
    \begin{tabular}{lp{5cm}}
        \toprule
        Label & Definition \\
        \midrule
        \textsc{added} & The label contains an \textbf{O}. \\
        \textsc{nonlinear} & An \textbf{A} is preceded by a \textbf{B}, or \textbf{X} or a \textbf{B} is followed by an \textbf{A} or \textbf{X}. \\
        \textsc{linear} & Both rules above are not met. \\
        \textsc{shared} & The label contains an \textbf{X}. \\
        \textsc{clipping} & One of the bases appears in its entirety, the other loses characters (this is a special case of linear blends). \todo{validate with data/code; alternately, this is just \say{a linear blend with no \textbf{X}}.} \\
        \textsc{boundary} & Either the rightmost or leftmost character is shared by more than one base (\textbf{X}). \\
        \textsc{insertion} & One base is properly contained within the other, whose characters occupy both the beginning and the end of the blend. \\
        \textsc{multi-base} & More than two bases are represented in the blend. \\
        \textsc{single-base} & A single base, blended with an affix. \\
        \bottomrule
    \end{tabular}
    \caption{Surface quality taxonomy. \todo{add counts}}
    \label{tab:surf_tags}
\end{table}

